3D Marketplace: Distributed Attestation of 3D Designs on Blockchain

Additive manufacturing (AM), or 3D printing, is an emerging manufacturing technology that is expected to have far-reaching socioeconomic, environmental, and geopolitical implications. As the use of this technology increases, the need for validation of 3D designs grows. In order to create a marketplace in which 3D designs are traded, it is necessary to develop a platform that enables the attestation of the 3D designs and promotes truthfulness. In this paper, we introduce a novel concept of a distributed marketplace that will support the attestation of 3D printing designs. We build a mathematical trust model that ensures truthfulness among rational, selfish, and independent agents, which is based on a reward/penalty system. The payment for participating in the evaluation is calculated by factoring in agents' reputation and peer feedback. Moreover, we describe the architecture and the implementation of the trust model on blockchain using smart contracts for the creation of a distributed marketplace. Our model relies both on theoretical and practical best practices to create an unique platform that elicit effort and truthfulness from the participants.

==> Conslusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we have presented a novel concept of a decentrelized marketplace that evaluates 3D designs and 
